Training Data Augmentation for Dysarthric Automatic Speech Recognition by Text-to-Dysarthric-Speech Synthesis

Automatic speech recognition (ASR) research has achieved impressive performance in recent years and has significant potential for enabling access for people with dysarthria (PwD) in augmentative and alternative communication (AAC) and home environment systems. However, progress in dysarthric ASR (DASR) has been limited by high variability in dysarthric speech and limited public availability of dysarthric training data. This paper demonstrates that data augmentation using text-to-dysarthic-speech (TTDS) synthesis for finetuning large ASR models is effective for DASR. Specifically, diffusion-based text-to-speech (TTS) models can produce speech samples similar to dysarthric speech that can be used as additional training data for fine-tuning ASR foundation models, in this case Whisper. Results show improved synthesis metrics and ASR performance for the proposed multi-speaker diffusion-based TTDS data augmentation for ASR fine-tuning compared to current DASR baselines.

==> discussion.tex <==
Notes on limitations: \newline
Data splits were created for the \emph{TORGO}, and utterances were randomly allocated. A systematic approach was considered, e.g.~considering the distribution of single/multi-word utterances, and distribution of utterances across splits. However, \cite{Yue2020}'s analysis shows there are $951$-$969$ unique utterances (across $16,158$ recordings), and not all dysarthric speakers completed recordings of all utterances. \textcolor{red}{Furthermore, there is an overlap of between $95.7$-$100\%$ in prompts in the \ac{LOSO} method}. Therefore, there were difficulties in determining an unbiased systematic method and random allocation was implemented. \newline
The results show that generally more data led to better metrics for \ac{TTDS}. However, there wasn't a significant difference in \ac{MCD} between \ac{SSp}, \ac{DSpG} and \ac{ASp} models. Experiments with further data will be required to establish this trend, and if potentially adaptation with more speakers with similar dysarthria severity is beneficial. \newline
Although the proposed system has increased \ac{WER} performance, further data and research is required to establish generalisation outside of the \emph{TORGO} \ac{ASR} task, particularly with out of vocabulary words due to overlapping prompts in the dataset. Also, there remains a gap in performance between mild to mod-severe, and severe dysarthric speakers. 

